MOSAIC: Modular Opinion Summarization using Aspect Identification and Clustering

Reviews are central to how travelers evaluate products on online marketplaces, yet existing summarization research often emphasizes end-to-end quality while overlooking benchmark reliability and the practical utility of granular insights. To address this, we propose MOSAIC, a scalable, modular framework designed for industrial deployment that decomposes summarization into interpretable components, including theme discovery, structured opinion extraction, and grounded summary generation. We validate the practical impact of our approach through online A/B tests on live product pages, showing that surfacing intermediate outputs improves customer experience and delivers measurable value even prior to full summarization deployment. We further conduct extensive offline experiments to demonstrate that MOSAIC achieves superior aspect coverage and faithfulness compared to strong baselines for summarization. Crucially, we introduce opinion clustering as a system-level component and show that it significantly enhances faithfulness, particularly under the noisy and redundant conditions typical of user reviews. Finally, we identify reliability limitations in the standard SPACE dataset and release a new open-source tour experience dataset (TRECS) to enable more robust evaluation.

==> app_TRECS.tex <==
\section{TRECS}
\label{section:trecs_appendix}

We constructed the TRECS dataset by applying MOSAIC to generate both theme-level summaries and product-level summaries from raw reviews, followed by human validation. Theme discovery and standardization were performed using GPT-4o-mini, while GPT-4.1-mini was used for both theme-constrained opinion extraction and opinion-aware review summarization. All generated theme and product summaries were then evaluated by a team of human annotators to ensure quality and consistency.
Table~\ref{tab:dataset_stats_TRECS} shows the distribution of top 10 themes in the data set.


\begin{table}[h]
\centering
\label{tab:theme_counts}
\begin{tabular}{l r}
\hline
\textbf{Theme} \& \textbf{Count} \\
\hline
Tour Guide or Instructors        & 320 \\
Tour Informativeness             & 287 \\
Tour Planning \& Coordination    & 252 \\
Point of Interest                & 237 \\
Natural Landscape Viewing        & 174 \\
Food \& Beverage                 & 172 \\
Driver                           & 169 \\
Tour Activities \& Participation & 160 \\
Value for Money                  & 110 \\
Tour Pacing                      & 110 \\
\hline
\end{tabular}
\caption{Distribution of top 10 themes in the dataset}
\label{tab:dataset_stats_TRECS}
\end{table}


==> app_opinion_redundancy_dataset.tex <==
\section{Opinion Redundancy Dataset}
\label{sec: opinion_redundancy_data_appendix}


To systematically evaluate the impact of opinion redundancy on theme-level opinion summarization, we constructed a controlled dataset that introduces varying levels and patterns of redundancy into opinion collections. Our dataset construction pipeline consists of four main stages:
\subsection{Cluster Quality Filtering}
\label{subsubsec: cluster_quality_filtering}
Following MOSAIC, we process reviews from a major travel experience platform and use the output of Section~\ref{subsubsec:opinion_clustering} (opinion clustering) as input to this stage. To ensure that only semantically coherent opinion groups are retained, we apply automated cluster quality filtering based on two complementary cohesion metrics:
\begin{itemize}[leftmargin=*]
    \item \textbf{Average distance from centroid} $\leq 0.2$, ensuring that opinions within a cluster are tightly concentrated around the centroid.
    \item \textbf{Average pairwise similarity} $\geq 0.7$, enforcing high inter-opinion coherence within each cluster.
\end{itemize}
Clusters failing either criterion are discarded. Filtering is performed at the \textit{Product-Theme-Sentiment} granularity, ensuring that subsequent sampling draws from high-quality, semantically consistent opinion groups.

\subsection{Diverse Opinion Sampling}
\label{subsubsec: diverse_opinion_sampling}
After identifying high-quality clusters, we consider the unclustered opinions within each \textit{Product–Theme–Sentiment} group, i.e., those not assigned to any HDBSCAN cluster. From this pool of unclustered opinions, we employ Maximal Marginal Relevance~\cite{carbonell1998use} sampling to select a diverse set of opinions. MMR balances two objectives:
\begin{itemize}[leftmargin=*]
    \item \textbf{Relevance}: Selecting opinions that are central to the theme.
    \item \textbf{Diversity}: Avoiding near-duplicate or semantically overlapping opinions.
\end{itemize}

Formally, the MMR score for an opinion $i$ is computed as:
\[
\text{MMR}(i) = (1 - \lambda)\,\text{Relevance}(i) - \lambda \max_{j \in S} \text{Similarity}(i, j),
\]
where $\lambda = 0.8$ controls the diversity-relevance trade-off, $S$ is the set of already selected opinions, relevance is defined as the mean cosine similarity of $i$ to all other opinions in the group, and similarity is the pairwise cosine similarity between opinion embeddings. Opinion embeddings are generated using the \texttt{all-MiniLM-L6-v2} sentence transformer. For each \textit{Product--Theme--Sentiment} group, we sample up to 10 opinions via MMR.


\subsection{Strategic Opinion Selection}
\label{subsubsec:strategic_opinion_selection}
To construct a fixed-size base opinion set for each \textit{Product--Theme--Sentiment} group, we combine opinions from two complementary sources:
\begin{itemize}[leftmargin=*]
    \item \textbf{Cluster representatives}: One opinion randomly selected from each high-quality cluster retained after cluster quality filtering (Section~\ref{subsubsec: cluster_quality_filtering}).
    \item \textbf{Diverse unclustered opinions}: Opinions sampled via Maximal Marginal Relevance (MMR) from the remaining unclustered opinion pool (Section~\ref{subsubsec: diverse_opinion_sampling}).
\end{itemize}

The selection process prioritizes cluster representatives to ensure that dominant semantic clusters are explicitly represented. If the number of cluster representatives is fewer than the target size, we fill the remaining slots using MMR-selected unclustered opinions, up to a maximum of 10 opinions per group. This strategy ensures that each \textit{Product--Theme--Sentiment} group contains exactly 10 base opinions, enabling controlled and systematic redundancy injection in subsequent stages.

\subsection{Redundancy Pattern Generation}
\label{subsubsec:redundancy_pattern_generation}

Given the fixed-size base opinion set of 10 opinions constructed for each \textit{Product--Theme--Sentiment} group (Section~\ref{subsubsec:strategic_opinion_selection}), we systematically introduce opinion redundancy by duplicating selected opinions within this set.

Specifically, we define 10 redundancy patterns, each represented by a duplication count vector
$\mathbf{c} = [c_1, c_2, \ldots, c_{10}]$, where $c_i$ denotes the number of times the $i$-th base opinion is repeated in the final input. The ordering of opinions follows the order established during strategic opinion selection, ensuring consistency across patterns.

Each redundancy pattern is designed to vary along 2 key dimensions: (i) redundancy intensity (ranging from moderate to extreme duplication), (ii) redundancy position (start, middle, end, or scattered within the opinion sequence) (see Table~\ref{tab:duplication_patterns}).

\begin{table}[t]
\centering
\small
\begin{tabular}{c c p{7.5cm}}
\hline
\textbf{Dataset Number} & \textbf{Duplication Vector} & \textbf{Description} \\
\hline
1  & {[}3000, 5, 5, 5, 5, 5, 5, 5, 5, 3000{]} & Extreme redundancy at boundaries \\
2  & {[}5, 5, 5, 3000, 3000, 5, 5, 5, 5, 5{]} & Extreme redundancy in the middle \\
3  & {[}3000, 3000, 5, 5, 5, 5, 5, 5, 5, 5{]} & Extreme redundancy at the start \\
4  & {[}3000, 5, 5, 3000, 5, 5, 5, 5, 5, 5{]} & Extreme redundancy scattered across positions \\
5  & {[}2000, 2000, 5, 5, 5, 5, 5, 5, 5, 2000{]} & High redundancy at boundaries \\
6  & {[}2000, 2000, 2000, 5, 5, 5, 5, 5, 5, 5{]} & High redundancy at the start \\
7  & {[}5, 5, 5, 5, 5, 5, 5, 2000, 2000, 2000{]} & High redundancy at the end \\
8  & {[}2000, 2000, 5, 5, 2000, 5, 5, 5, 5, 5{]} & High redundancy scattered across positions \\
9  & {[}5, 5, 5, 5, 2000, 5, 5, 5, 2000, 2000{]} & High redundancy at end positions \\
10 & {[}1000, 1000, 1000, 1000, 5, 5, 5, 5, 5, 2000{]} & Mixed redundancy levels \\
\hline
\end{tabular}
\caption{Synthetic redundancy patterns used to construct high-redundancy evaluation datasets. Each duplication vector specifies how many times each of the ten base opinions is repeated.}
\label{tab:duplication_patterns}
\end{table}

For each \textit{Product--Theme--Sentiment} group, we generate 10 dataset variants-one per redundancy pattern resulting in controlled inputs that isolate the effects of redundancy intensity, position, and distribution on downstream summarization performance.

==> app_space_dataset_results.tex <==
\section{Results on SPACE Dataset}
\label{subsec: space_dataset_results}
\noindent\textbf{SPACE (Table \ref{tab:space_comparison_table})}. Under GPT-4o, both methods achieve identical Coverage and G-Eval, while \cite{li2025decomposed} attains slightly higher AlignScore-R/M. 
This trend reverses for Llama-70B, where our method improves Coverage and yields sizeable relative gains in AlignScore-R ($\sim$7–8\%) and AlignScore-M ($\sim$45\%), demonstrating stronger factual consistency under a weaker base model.
\begin{table*}[ht]
\centering
\footnotesize
\begin{tabular}{lcccc}
\hline
\textbf{Methods} & \textbf{Coverage$\uparrow$} & \textbf{G-Eval$\uparrow$} & \textbf{AlignScore-R/M$\uparrow$}\\
\hline
HIRO-abs \cite{hosking2024hierarchical} & 0.87 & 0.62 & \underline{0.83}/\underline{\textbf{0.24}}\\
TCG \cite{bhaskar2022prompted} & 0.98 & 0.66 & 0.66/0.11\\
Aspect-aware decomposition-GPT-4o \cite{li2025decomposed} & \underline{\textbf{1.00}} & \underline{\textbf{0.90}} & 0.81/0.10\\
MOSAIC GPT-4o (ours) & \underline{\textbf{1.00}} & \underline{\textbf{0.90}} & 0.77/0.07\\
\hline
Automatic decomposition-Llama 70B \cite{khot2022decomposed} & 0.63 & 0.38 & 0.70/\underline{0.22}\\
Chunk-wise decomposition-Llama 70B \cite{khot2022decomposed} & 0.93 & 0.84 & 0.65/0.01\\
Naive aspect-aware prompting-Llama 70B \cite{radford2019language} & 0.37 & 0.34 & 0.44/\underline{0.22}\\
Aspect-aware decomposition-Llama 70B \cite{li2025decomposed} & \underline{0.99} & \underline{0.88} & 0.79/0.11\\
MOSAIC-Llama 70B (ours) & \underline{0.99} & \underline{0.88} & \textbf{0.86}/0.16\\
\hline
\end{tabular}

\vspace{2mm}
\caption{Results on SPACE - The first section of the table presents results for GPT-4o and state-of-the-art models. The second section has results for Llama 70B. Underlined scores denote best in section per metric, while bold scores denote best overall. AlignScore-R calculates AlignScore against source reviews, while AlignScore-M is computed against reference meta-reviews.}
\label{tab:space_comparison_table}
\end{table*}

==> intro.tex <==
\section{Introduction}


Online reviews are a key resource for purchase decisions, as they provide authentic signals of product and service quality \cite{boorugu2020survey}. Automatic opinion summarization seeks to condense large and diverse sets of reviews for a given entity into a concise, readable meta-summary. 
An effective summary should capture dominant opinions, include user-relevant aspects, and remain grounded in supporting evidence. In practice, users may seek either a product-level overview or theme-specific summaries focused on particular aspects. For tour-related products, this may include the quality of the tour guide, the convenience of the pickup location, or whether the food meets user expectations. 
Summaries should therefore remain balanced and focus only on themes that matter to users in general. 
\begin{comment}
In addition, review sets for popular products can exceed the effective context window of current models, further increasing the risk of factual errors, as demonstrated in multiple long-context summarization applications (Kim et al., 2024; Bai et al., 2024; Liu et al., 2024)
\end{comment}

\cite{bhaskar2022prompted} proved that prompted LLMs produce faithful summaries for short inputs (under 1,000 words), but repeated summarization on longer inputs leads to increasingly generalized and less faithful outputs\todo[inline]{maybe it will be better to mention the models they worked with, because back in 2022 maybe some recent models might not be present, and that was their constraint with shorter context size}.

\cite{tang2024prompted} proposed a fully automated aspect extraction approach through few-shot prompting but their summaries are harder to validate without grounding evidence\todo{I think we should elaborate this a bit more mentioning the exact reason why was not possible}.

Talk about opinion summarisation and the importance of it?
\cite{hosking2023attributable} - this paper coined the term ``opinion summarisation''

\cite{zeng2024scientific} -
\cite{amplayo2021aspect} - talks about opinion summarisation

\cite{zeng2024scientific}- ORSUM data set. read about it

\cite{li2024sentiment}- this paper proposed the approach of splitting the process into 3 parts - extraction (similar to absa output), regroup opinions and then use it for summary. this paper proved that this way of dividing the process make summaries more faithful.

We took inspiration from recent applications of chain-of-thought prompting \cite{wei2022chain} and its variants (Khot et al., 2023; Zhou
et al., 2023), which address reasoning problems
by decomposing complex tasks into a sequence of
simpler sub-problems, which are solved sequentially. \cite{li2025decomposed} propose a great opinion summarization framework but do not address large-scale theme extraction or opinion redundancy.


``Bhaskar et al. (2023) and Li et al. (2024)
use similar modules to ours. However, intermediate results of their recursive prompting and aspect
identification are not inspected or verified and there
is limited transparency, and Li et al. (2024) focus
exclusively aspects in scientific reviews (e.g., opinions about Novelty or Soundness).''
\todo[inline]{this is where history of past experiment ends}


In this paper, we propose an end to end framework from theme extraction at scale to using the output for review summarisation.
Our approach consists of three high level modules- \textit{Theme Discovery \&w Standardization}, \textit{Theme-Constrained Opinion Extraction} and \textit{Opinion-Aware Review Summarization}. 
We first identify relevant themes using a few-shot LLM-based approach and refine them through human review to ensure user relevance. These themes are then used to extract structured ABSA\todo{ABSA is not introduced before} outputs—covering theme, aspect, opinion, and sentiment via LLMs. To address opinion redundancy, we apply opinion clustering before generating theme-level summaries, which are subsequently composed into product-level summaries. Human evaluations show that our approach produces higher-quality and more faithful summaries.
Our main contributions are as follows:\todo{re-wording contributions}
\begin{itemize}
    \item We propose a scalable, end-to-end framework for review summarization that integrates large-scale theme discovery, structured opinion extraction, and human-in-the-loop validation.
    \item We introduce opinion clustering as a key component of opinion summarization and empirically demonstrate its impact on improving summary faithfulness.
    \item We release a first-of-its-kind open-sourced dataset of travel experiences, containing 344 products, roughly 14k reviews, annotated themes, and generated summaries at both the product and theme levels.
    \item We further showcase real-world industrial use cases of the framework, highlighting its ability to deliver a more granular and transparent user experience.
\end{itemize}
\todo[inline]{AB test screenshot Viator}
\todo[inline]{code to be released}

==> open_source_dataset.tex <==
% \section{Real World Dataset}
% To support further research in opinion summarization, we release a dataset from the travel-experience domain. 
% The dataset comprises 344 products with a total of 140,631 reviews, with an average review length of XX characters and approximately 400 reviews per product. 
% For each product, we identify eight frequently discussed themes extracted from the reviews. 
% Opinions associated with these themes are used to generate theme-level summaries, and the same set of themes is leveraged to produce product-level summaries. 
% This design provides a unified and consistent representation across theme and product summaries, and directly addresses the gap identified in Section X.
% These summaries have been verified by a team of 4 people with 

==> problem_formulaton.tex <==
\section{Problem Formulation}

Let $R_{p} = \{r_1, r_2, \ldots, r_n\}$ denote a corpus of user reviews associated with a product $p$ from a domain $d$ (e.g., hotels or travel experiences). 
Reviews in $R_{p}$ may discuss multiple themes drawn from a domain-specific theme set
$\mathcal{T}_d = \{t_1, t_2, \ldots, t_m\}$, such as tour guide, pickup logistics, or food.

Each review $r_j \in R_{p}$ may express opinions on one or more themes in $\mathcal{T}_d$. For a given theme $t_i$, let
\[
R_{p, t_i} = \{ r_j \in R_p \mid r_j \text{ contains opinions related to } t_i \}
\]
denote the subset of reviews relevant to that theme. 
We decompose the task into three modules, namely Theme Discovery \& Standardization, Theme-Constrained Opinion Extraction, and Opinion-Aware Review Summarization.
\todoj{We need to say something more here, otherwise it is incomplete, as we name this section as problem formulation. JC todo. Or the question is do we need this section?}
